A Power Analysis of the Conditional Randomization Test and Knockoffs

In many scientific problems, researchers try to relate a response variable $Y$ to a set of potential explanatory variables $X = (X_1,\dots,X_p)$, and start by trying to identify variables that contribute to this relationship. In statistical terms, this goal can be posed as trying to identify $X_j$'s upon which $Y$ is conditionally dependent. Sometimes it is of value to simultaneously test for each $j$, which is more commonly known as variable selection. The conditional randomization test (CRT) and model-X knockoffs are two recently proposed methods that respectively perform conditional independence testing and variable selection by, for each $X_j$, computing any test statistic on the data and assessing that test statistic's significance by comparing it to test statistics computed on synthetic variables generated using knowledge of $X$'s distribution. Our main contribution is to analyze their power in a high-dimensional linear model where the ratio of the dimension $p$ and the sample size $n$ converge to a positive constant. We give explicit expressions of the asymptotic power of the CRT, variable selection with CRT $p$-values, and model-X knockoffs, each with a test statistic based on either the marginal covariance, the least squares coefficient, or the lasso. One useful application of our analysis is the direct theoretical comparison of the asymptotic powers of variable selection with CRT $p$-values and model-X knockoffs; in the instances with independent covariates that we consider, the CRT provably dominates knockoffs. We also analyze the power gain from using unlabeled data in the CRT when limited knowledge of $X$'s distribution is available, and the power of the CRT when samples are collected retrospectively.

==> appendices/knockoffs.tex <==
\section{Quality of the knockoffs}
\label{sec:knock-qual}
It has been observed and noted that the quality of the knockoffs plays an important role its performance \citep{candes2018panning,SB-EC-LJ-WW:2020}. In this section, we discuss how the quality of the knockoffs affects power. We focus on the correlation between the covariates and their knockoff counterparts, as suggested in \citet{candes2018panning}. It should be clear from the previous section that in order to achieve high power, the non-null $p$-values should have very different distributions than the null $p$-values. To better understand the mechanism, consider %a toy setting where we have $p$ independent statistic $T_j\sim\mathcal N(\theta_j,1)$, with $\gamma$ fraction of $\theta_j$'s being $0$ and $(1-\gamma)$ being $h$. Suppose we have knockoff statistics $T_{j+p}$ from $\mathcal N(0,1)$, jointly normal with $T_j$ with correlation $\rho$ and independent of the other $T_j$'s. This can be thought of as
a linear regression case where each non-null $\beta_j=h/\sqrt{n}$, the error variance is $1$, $n\gg p$, and independently for each $j$ we have
\begin{equation*}
\left(
  \begin{array}{c}
X_j\\
\tilde X_j\\
  \end{array}
\right)\sim\mathcal N\left(\left(
  \begin{array}{c}
0\\
0\\
  \end{array}
\right),\left[
  \begin{array}{cc}
1 & -\rho\\
-\rho & 1\\
  \end{array}
\right]\right).
\end{equation*}
Suppose we let the variable importance statistic be $W_j=\sqrt n(|\hat\beta_j|-|\hat\beta_{j+p}|)$. If we let $F_{\mu,\rho}$ be the distribution of $|X|-|Y|$, where
\begin{equation*}
\left(
  \begin{array}{c}
X\\
Y\\
  \end{array}
\right)\sim\mathcal N\left(\left(
  \begin{array}{c}
\mu\\
0\\
  \end{array}
\right),\left[
  \begin{array}{cc}
1 & \rho\\
\rho & 1\\
  \end{array}
\right]\right),
\end{equation*}
then it can be seen that the null $W_j=\sqrt n(\hat\beta_j-\hat\beta_{j+p})$ has distribution $(1-\rho^2)^{-1/2}F_{0,\rho}$, and the non-null $W_j$ has distribution $(1-\rho^2)^{-1/2}F_{h\sqrt{1-\rho^2},\rho}$. = Intuitively, we can expect high power if $F_{h\sqrt{1-\rho^2},\rho}$ is quite different from $(1-\rho^2)^{-1/2}F_{0,\rho}$, which should occur when $|\rho|$ is low. In Figure~\ref{fig:compare-rhos}, we compare the two distributions for different $\rho$. The two distributions become more entangled as $\rho$ grows, while the change is flat when $\rho$ is small.

Note that
\begin{equation*}
\begin{aligned}
F_{\mu,\rho}(x)&=1-\p(\{X-Y\ge x,X+Y\ge x\}\cup\{X+Y\le-x,X-Y\le-x\})\\
&=1-\p(X-Y\ge x,X+Y\ge x)-\p(X+Y\le-x,X-Y\le-x)\\
&\quad+\p(X-Y\ge x,X+Y\ge x,X+Y\le-x,X-Y\le-x)\\
&=1-\Phi(\frac{\mu-x}{\sqrt{2(1+\rho)}})\Phi(\frac{\mu-x}{\sqrt{2(1-\rho)}})-\Phi(\frac{-\mu-x}{\sqrt{2(1+\rho)}})\Phi(\frac{-\mu-x}{\sqrt{2(1-\rho)}})\\
&\quad+\mathbb I(x<0)\left[\Phi(\frac{-x-\mu}{\sqrt{2(1+\rho)}})-\Phi(\frac{x-\mu}{\sqrt{2(1+\rho)}})\right]\left[\Phi(\frac{-x-\mu}{\sqrt{2(1-\rho)}})-\Phi(\frac{x-\mu}{\sqrt{2(1-\rho)}})\right].
\end{aligned}
\end{equation*}

% Let
% \begin{equation*}
% \begin{aligned}
% \tau_\text{KF}&=\min\{t>0:\frac{1+\#\{j:W_j\le-t\}}{\#\{j:W_j\ge t\}}\ge q\}\\
% &\approx\min\{t>0:\frac{\gamma F_{0,\rho}(-t)+(1-\gamma)F_{h\sqrt{n(1-\rho^2)},\rho}(-t)}{\gamma F_{0,\rho}(-t)+(1-\gamma)(1-F_{h\sqrt{n(1-\rho^2)},\rho}(t))}\le q\},
% \end{aligned}
% \end{equation*}
% and the power is $1-F_{h\sqrt{n(1-\rho^2)},\rho}(\tau_\text{KF})$.

\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/rho/rho0.pdf}
         \caption{$\rho=0$}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/rho/{rho0.2}.pdf}
         \caption{$\rho=0.2$}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/rho/{rho0.4}.pdf}
         \caption{$\rho=0.4$}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/rho/{rho0.6}.pdf}
         \caption{$\rho=0.6$}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/rho/{rho0.8}.pdf}
         \caption{$\rho=0.8$}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/rho/{rho0.99}.pdf}
         \caption{$\rho=0.99$}
     \end{subfigure}
        \caption{Comparison of $(1-\rho^2)^{-1/2}F_{h\sqrt{1-\rho^2},\rho}$ (black) and $F_{0,\rho}$ (blue) with $h=3$.}
        \label{fig:compare-rhos}
\end{figure}
